$\widetilde{\tau}$ searches at future e$^+$e$^-$ colliders

The direct pair-production of the superpartner of the $\tau$-lepton, the $\widetilde{\tau}$, is one of the most interesting channels to search for SUSY in: the $\widetilde{\tau}$ is likely to be the lightest of the scalar leptons, and is one of the most experimentally chalanging ones. The current model-independent $\widetilde{\tau}$ limits come from LEP, while limits obtained at the LHC do extend to higher masses, but are model-dependent. The future Higgs factories will be powerful facilities for SUSY searches, offering advantages with respect to previous electron-positron colliders as well as to hadron machines. In order to quantify the capabilities of these future $e^+e^-$ colliders, the "worst-case" scenario for $\widetilde{\tau}$ exclusion/discovery has been studied, taking into account the effect of the $\widetilde{\tau}$ mixing on $\widetilde{\tau}$ production cross-section and detection efficiency. To evaluate the latter, the ILD concept, originally developed for the International Linear Collider (ILC), and the ILC beam conditions at a centre-of-mass energy of 500 GeV have been used for detailed simulations. The obtained exclusion and discovery reaches extend to only a few GeV below the kinematic limit even in the worst-case scenario. The results of the detailed simulation study are then discussed in view of the experimental environment of other proposed Higgs factory projects.

==> references.tex <==
\begin{thebibliography}{99}
  \itemsep0.5ex
  
%\cite{Curtin:2014cca}
\bibitem{Curtin:2014cca}
D.~Curtin, R.~Essig, S.~Gori and J.~Shelton,
%``Illuminating Dark Photons with High-Energy Colliders,''
JHEP \textbf{02} (2015), 157
%doi:10.1007/JHEP02(2015)157
\href{https://arxiv.org/abs/1412.0018}{[arXiv:1412.0018 [hep-ph]]}.
%340 citations counted in INSPIRE as of 22 Oct 2023

\bibitem{EuropeanStrategyforParticlePhysicsPreparatoryGroup:2019qin}
  R.~K.~Ellis,  \textit{et al.}
%R.~K.~Ellis, B.~Heinemann, J.~de Blas, M.~Cepeda, C.~Grojean, F.~Maltoni, A.~Nisati, E.~Petit, R.~Rattazzi and W.~Verkerke, \textit{et al.}
%``Physics Briefing Book: Input for the European Strategy for Particle Physics Update 2020,''
CERN-ESU-004, \href{https://arxiv.org/abs/1910.11775}{[arXiv:1910.11775 [hep-ex]]}.
% 120 citations counted in INSPIRE as of 02 Nov 2021

%\cite{Karliner:2015tga}
\bibitem{Karliner:2015tga}
M.~Karliner, M.~Low, J.~L.~Rosner and L.~T.~Wang,
%``Radiative return capabilities of a high-energy, high-luminosity $e^+e^-$ collider,''
Phys. Rev. D \textbf{92} (2015) no.3, 035010
%doi:10.1103/PhysRevD.92.035010
\href{https://arxiv.org/abs/1503.0720}{[arXiv:1503.07209 [hep-ph]]}.
%28 citations counted in INSPIRE as of 22 Oct 2023


%\cite{Behnke:2013xla}
\bibitem{Behnke:2013xla}
  T.~Behnke, J.~E.~Brau, B.~Foster, \textit{et al.},
  %J.~Fuster, M.~Harrison, J.~M.~Paterson, M.~Peskin, M.~Stanitzki, N.~Walker and H.~Yamamoto,
%``The International Linear Collider Technical Design Report - Volume 1: Executive Summary,''
\href{https://arxiv.org/abs/1306.6327}{[arXiv:1306.6327 [physics.acc-ph]]}.
% 625 citations counted in INSPIRE as of 22 Oct 2023

%\cite{Vernieri:2022fae}
\bibitem{Vernieri:2022fae}
  C.~Vernieri, E.~A.~Nanni, S.~Dasu, \textit{et al.},
  %, M.~E.~Peskin, T.~Barklow, K.~Agashe, R.~Bartoldus, P.~C.~Bhat, K.~Black and J.~E.~Brau, \textit{et al.}
%``Strategy for Understanding the Higgs Physics: The Cool Copper Collider,''
JINST \textbf{18} (2023) no.07, P07053
%doi:10.1088/1748-0221/18/07/P07053
\href{https://arxiv.org/abs/2203.07646}{[arXiv:2203.07646 [hep-ex]]}.
% 30 citations counted in INSPIRE as of 22 Oct 2023

%\cite{Linssen:2012hp}
\bibitem{Linssen:2012hp}
L.~Linssen, A.~Miyamoto, M.~Stanitzki and H.~Weerts,
%``Physics and Detectors at CLIC: CLIC Conceptual Design Report,''
%doi:10.5170/CERN-2012-003
\href{https://arxiv.org/abs/1202.5940}{[arXiv:1202.5940 [physics.ins-det]]}.
%557 citations counted in INSPIRE as of 22 Oct 2023

%\cite{CEPCStudyGroup:2018rmc}
\bibitem{CEPCStudyGroup:2018rmc}
 [CEPC Study Group],
%``CEPC Conceptual Design Report: Volume 1 - Accelerator,''
\href{https://arxiv.org/abs/1809.00285}{[arXiv:1809.00285 [physics.acc-ph]]}.
% 373 citations counted in INSPIRE as of 22 Oct 2023

%\cite{FCC:2018evy}
\bibitem{FCC:2018evy}
A.~Abada \textit{et al.} [FCC],
%``FCC-ee: The Lepton Collider: Future Circular Collider Conceptual Design Report Volume 2,''
Eur. Phys. J. ST \textbf{228} (2019) no.2, 261-623
%doi:10.1140/epjst/e2019-900045-4
% 864 citations counted in INSPIRE as of 22 Oct 2023

%\cite{ILDConceptGroup:2020sfq}
\bibitem{ILDConceptGroup:2020sfq}
H.~Abramowicz \textit{et al.} [ILD Concept Group],
%``International Large Detector: Interim Design Report,''
\href{https://arxiv.org/abs/2003.01116}{[arXiv:2003.01116 [physics.ins-det]]}.
% 103 citations counted in INSPIRE as of 22 Oct 2023


%\cite{Kilian:2007gr}
\bibitem{Kilian:2007gr}
W.~Kilian, T.~Ohl and J.~Reuter,
%``WHIZARD: Simulating Multi-Particle Processes at LHC and ILC,''
Eur. Phys. J. C \textbf{71} (2011), 1742
%doi:10.1140/epjc/s10052-011-1742-y
\href{https://arxiv.org/abs/0708.4233}{[arXiv:0708.4233 [hep-ph]]}.
%862 citations counted in INSPIRE as of 22 Oct 2023



\end{thebibliography}

